An ExpTime Upper Bound for $\mathcal{ALC}$ with Integers (Extended Version)

Concrete domains, especially those that allow to compare features with numeric values, have long been recognized as a very desirable extension of description logics (DLs), and significant efforts have been invested into adding them to usual DLs while keeping the complexity of reasoning in check. For expressive DLs and in the presence of general TBoxes, for standard reasoning tasks like consistency, the most general decidability results are for the so-called $\omega$-admissible domains, which are required to be dense. Supporting non-dense domains for features that range over integers or natural numbers remained largely open, despite often being singled out as a highly desirable extension. The decidability of some extensions of $\mathcal{ALC}$ with non-dense domains has been shown, but existing results rely on powerful machinery that does not allow to infer any elementary bounds on the complexity of the problem. In this paper, we study an extension of $\mathcal{ALC}$ with a rich integer domain that allows for comparisons (between features, and between features and constants coded in unary), and prove that consistency can be solved using automata-theoretic techniques in single exponential time, and thus has no higher worst-case complexity than standard $\mathcal{ALC}$. Our upper bounds apply to some extensions of DLs with concrete domains known from the literature, support general TBoxes, and allow for comparing values along paths of ordinary (not necessarily functional) roles.

==> 3-automata.tex <==
\section{Embeddability and Automata}

Assume we have degree $n$.
\begin{definition}[Rabin tree automaton]
\label{def_Rabin_tree_automaton}
A \emph{Rabin tree automaton} over the alphabet $\Sigma$ has the form $\cA = (Q, q_0, \longrightarrow, \Omega)$ 
with a finite state set $Q$, initial state $q_0$, transition relation $\longrightarrow \subseteq Q \times A \times Q^n$,
and $\Omega = \{(L_1,U_1), \ldots, (L_m,U_m)\}$ is a collection of ``accepting pairs'' of state sets $L_i, U_i \subseteq Q$.
A \emph{run} of $\cA$ on a tree $T$ is a map $r : \{0,\ldots,n\}^\star \rightarrow Q$ with $r(\varepsilon) = q_0$
and $(r(w),T(w),r(w0),\ldots,r(wn)) \in \longrightarrow$ for $w \in \{0,\ldots,n\}^\star$.
A run $r$ of the Rabin automaton $\cA$ is \emph{successful} if 
\begin{center}
	for all paths $\pi$ there exists an $i \in \{1, \ldots, m\}$ with \\
	$\mathrm{In}(r \mid \pi) \cap L_i = \emptyset$ and $\mathrm{In}(r \mid \pi) \cap U_i \neq \emptyset$.
\end{center}
A tree $T$ is \emph{accepted} by the Rabin tree automaton if some run of $\cA$ in $T$ is successful.
\end{definition}


\begin{definition}
\label{def_rooted_subtree}
For a tree $T$ over $\Sigma$, the \emph{subtree rooted at $w \in \Sigma^\star$} is the tree $\left.T\right|_{w}(v) = T(wv)$
for all $v \in \Sigma^\star$.  
\end{definition}

\begin{definition}[Regular tree]
\label{def_regular_tree}
We say that a tree $T$ over $\Sigma$ is \emph{regular} if the set 
$\{\left. T \right|_{u} \mid u \in \Sigma^\star\}$ of subtrees of $T$ is finite up to isomorphism.
Equivalently, $T$ is regular if there is a finite automaton $\mathcal{A}$ over words whose state set is partitioned into sets $Q_a (a \in \Sigma)$
such that $\mathcal{A}$ reaches a state in $Q_a$ via input $u$ iff $T(u) = a$.
\end{definition}


\begin{theorem}[Rabin's Theorem \cite{bk_rabin72}]
Any non-empty Rabin recognizable set of trees contains a regular tree.
\end{theorem}
As a consequence of this theorem, it will be enough to find a condition for embeddability which is necessary and sufficient for regular trees,
which is verifiable by a Rabin tree automaton.

\subsection{Embeddability condition for regular trees}

We actually give the condition on the constraint graph.
We describe how constraint graphs for tree models can be represented as trees. 

\begin{definition}[forward path, backward path]
\label{def_forward_path}
\label{def_backward_path}
An infinite path $p : \mathbb{N} \rightarrow \Delta \times \mathsf{Reg}$ is a \emph{forward path}
if for every $n \in \mathbb{N}$, there is an edge from $p(i)$ to $p(i+1)$. 
It is a \emph{backward path} if for every $n \in \mathbb{N}$, there is an edge from $p(i+1)$ to $p(i)$.
\end{definition}


\begin{description}
\item[Condition (on the framified constraint graph)]
There are no $u.x,u.y \in \Delta \times \mathsf{Reg}$ in $\mathcal{G}_{\mathrm{fr}}$ 
for which the following holds. There is an infinite $\mathbf{w} \in \Delta^\omega$ and
\begin{enumerate}
	\item 
	an infinite forward downward path $f$ from $u.x$ along $\mathbf{w}$
	\item
	an infinite backward downward path $b$ from $u.v$ along $\mathbf{w}$
\end{enumerate}
such that $f$ or $b$ is strict, and such that for every $i \in \mathbb{N}$, there is a strict edge from $f(i)$ to $b(i)$.
\end{description}
Note that this condition is on constraint graphs, not trees.


\subsection{A Rabin tree automaton for embeddability}

We describe a Rabin tree automaton $\cB$ which runs on trees over an alphabet of frames, that satisfy certain consistency conditions.
This automaton finds a bad pair of registers, i.e., if $\cB$ accepts the tree, the constraint graph corresponding to it is not embeddable.
Then the desired automaton $\cA_{\mathrm{emb}}$ is the complement of $\cB$.

We first describe the alphabet of frames.
The registers we have are $\mathsf{Reg}_\rho = \{x_1,\ldots, x_\rho\}$.
Denote $\mathsf{Reg}_\rho^{\mathrm{top}} = \{x_1^{\mathrm{top}},\ldots, x_\rho^{\mathrm{top}}\}$,
and $\mathsf{Reg}_\rho^{\mathrm{bot}} = \{x_1^{\mathrm{bot}},\ldots, x_\rho^{\mathrm{bot}}\}$.

\begin{definition}[Frame]
\label{def_frame}
A frame is a directed graph with labeled edges where
$V = \mathsf{Reg}_\rho^{\mathrm{top}} \cup \mathsf{Reg}_\rho^{\mathrm{bot}}$ and $E = E_{<} \cup E_{=}$
and
\begin{enumerate}
	\item 
	there is an edge between every pair of vertices
	\item
	if $e_=(x,y)$ then also $e_=(y,x)$
	\item
	there are no strict cycles
\end{enumerate}


\end{definition}


\paragraph*{Description of the automaton}
We begin by saying that the problematic pair is (a) in the current subtree (b) but not the current node ($q_0$). 
Then we pick one child for which (a) is also true and possibly also (b), the other children go into a state meaning the problematic pair in not
in the subtree ($q_1$). 

At some point, we move from state $q_0$ to a state where we guess the problematic pair and whether
it is the forward path $f$ or the backward path $b$ which will be strict. This is indicated with a flag $f$ or $b$ which does not
change once chosen. We have another flag $0/1$ indicating whether we just witnessed a strict edge. Call these path states.

Every step, we chose a child with which the path continues which is labeled with a path state where we guess how the path continues.
Other children are labeled with $q_1$.

We must witness a $1$ flag for strictness infinitely often.


Define $\mathcal{B} = (Q, q_0, \longrightarrow, (\emptyset, U))$ over the alphabet of frames.
Assume we have degree $k$.

\begin{itemize}
	\item
	$Q = \{q_0,q_1,q_2\} \cup \mathsf{Reg}_\rho \times \mathsf{Reg}_\rho \times \{f,b \} \times \{ 0,1\}$
	\begin{itemize}
		\item 
		$q_2$ means that the problem pair will be guessed to be in the current subtree but not the current node.
		\item
		$q_1$ means the problem pair will not be guessed to be in the current subtree.
		\item
		The other states specify which pair of registers extends the path, whether it is the forward or the backward path that is strict, and whether
		we have just witnessed a strict edge in the relevant direction
	\end{itemize}
	\item
	$U = \{q_1\} \cup \mathsf{Reg}_\rho \times \mathsf{Reg}_\rho \times \{f,b \} \times \{1\}$
	\item
	$\longrightarrow$ is given as follows.
	Denote by $\mathbf{q}^e_i$ the $k$-tuple containing $q_2$ for entry $i$
			and $q_1$ for every other entry.
	\begin{itemize}
		\item 
		For every $i \in \{1, \ldots, k\}$, we have 
		$q_0 \overset{v}{\longrightarrow} \mathbf{q}^e_i$ and
		$q_2 \overset{v}{\longrightarrow} \mathbf{q}^e_i$ 
		\item
		$q_1 \overset{v}{\longrightarrow} (q_1, \ldots, q_1)$ 
	\end{itemize}	
	For every $i \in \{1, \ldots, k\}$, $h \in \{f,b\}$, and $- \in \{0,1\}$ denote by $(x, y, h , - )_i$ the $k$-tuple containing $(x, y, h , -)$ for entry $i$
		and $q_1$ for every other entry.
		\begin{itemize}
			\item
		For every $i \in \{1, \ldots, k\}$ and $h \in \{f,b\}$
		we have 
		$q_0 \overset{v}{\longrightarrow} (x,y,h,0)_i$
		and
		$q_2 \overset{v}{\longrightarrow} (x,y,h,0)_i$
		if $e_<(x^{\mathrm{bot}},y^{\mathrm{bot}}) \in v$
		
		\end{itemize}
		We describe the transitions for the case where we guessed that the forward path is strict.
		\begin{itemize}
		\item
		For every $i \in \{1, \ldots, k\}$, we have
		\[
		(x,y,f,-) \overset{v}{\longrightarrow} \mathbf{(} z, w, f ,1 \mathbf{)}_i
		\]
		if we have
		\begin{enumerate}
			\item 
			$e_<(x^{\mathrm{top}},z^{\mathrm{bot}}) \in v$
			\item
			$e_<(x^{\mathrm{top}},y^{\mathrm{top}}) \in v$
			\item
			$e_<(z^{\mathrm{bot}},w^{\mathrm{bot}}) \in v$
			\item
			$e_<(y^{\mathrm{top}},w^{\mathrm{bot}}) \notin v$
		\end{enumerate}
		
		\item
		
		Similarly, if the current edge on the forward path is not strict, 
		i.e.\
		if we have
		\begin{enumerate}
			\item 
			$e_=(x^{\mathrm{top}},z^{\mathrm{bot}}) \in v$
			\item
			$e_<(x^{\mathrm{top}},y^{\mathrm{top}}) \in v$
			\item
			$e_<(z^{\mathrm{bot}},w^{\mathrm{bot}}) \in v$
			\item
			$e_<(y^{\mathrm{top}},w^{\mathrm{bot}}) \notin v$
		\end{enumerate}
		then we have
		\[
		(x,y,f,-) \overset{v}{\longrightarrow} \mathbf{(} z, w, f ,0 \mathbf{)}_i
		\] 
		\item		
		We have similar transitions for the case where we guessed that the backward path is strict.
	\end{itemize}
\end{itemize}
The automaton $\mathcal{A}_{\mathrm{emb}}$ is the complement of $\mathcal{B}$, 
it may have exponentially many more states than $\mathcal{B}$ \cite{ar_MullerSchupp95}.

